Fast and parallel decoding for transducer

The transducer architecture is becoming increasingly popular in the field of speech recognition, because it is naturally streaming as well as high in accuracy. One of the drawbacks of transducer is that it is difficult to decode in a fast and parallel way due to an unconstrained number of symbols that can be emitted per time step. In this work, we introduce a constrained version of transducer loss to learn strictly monotonic alignments between the sequences; we also improve the standard greedy search and beam search algorithms by limiting the number of symbols that can be emitted per time step in transducer decoding, making it more efficient to decode in parallel with batches. Furthermore, we propose an finite state automaton-based (FSA) parallel beam search algorithm that can run with graphs on GPU efficiently. The experiment results show that we achieve slight word error rate (WER) improvement as well as significant speedup in decoding. Our work is open-sourced and publicly available\footnote{https://github.com/k2-fsa/icefall}.

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Dataset and Setup}
The Librispeech corpus~\cite{librispeech2015}, which contains 970 hours
of audiobook data with corresponding text transcripts, is used for ASR training.
We extract 80-channel log
Mel-filter bank values from a 25ms window with a stride of 10ms to produce
the acoustic feature frames. To prevent overfitting and to improve generalization,
frequency masking (F = 27, mF = 2) and time masking (T = 100, mT = 2) are applied
during model training according to~\cite{park2019specaug}. We also use
noise augmentation by randomly mixing the noise audios from MUSAN~\cite{musan2015}
into the training data with an SNR ranging from 10 to 20. Furthermore, speed
perturbation~\cite{ko2015audio} with factors 0.9 and 1.1 is used to triple
the training set.

The encoder model is a Conformer~\cite{anmol2020conformer} model
with 12 encoder layers, each of which contains 8 self-attention~\cite{vaswani2017attention}
heads with attention-dim 512.
The subsampling factor in the convolution module is 4 and the feed-forward
dimension is 2048. The decoder model is a stateless network~\cite{ghodsi2020rnntstateless},
consisting of an embedding layer with embedding dimension 512 followed by a 1-D
convolution layer with kernel size 2. The number of output units is
500 BPE~\cite{kudo-richardson-2018-sentencepiece} tokens.
%
The code is open-sourced and publicly available at
\url{https://github.com/k2-fsa/icefall}.
